Efficient Tensor Kernel methods for sparse regression

Recently, classical kernel methods have been extended by the introduction of suitable tensor kernels so to promote sparsity in the solution of the underlying regression problem. Indeed, they solve an lp-norm regularization problem, with p=m/(m-1) and m even integer, which happens to be close to a lasso problem. However, a major drawback of the method is that storing tensors requires a considerable amount of memory, ultimately limiting its applicability. In this work we address this problem by proposing two advances. First, we directly reduce the memory requirement, by intriducing a new and more efficient layout for storing the data. Second, we use a Nystrom-type subsampling approach, which allows for a training phase with a smaller number of data points, so to reduce the computational cost. Experiments, both on synthetic and read datasets, show the effectiveness of the proposed improvements. Finally, we take case of implementing the cose in C++ so to further speed-up the computation.

==> frontespizio.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TITOLO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagenumbering{Alph}
\begin{titlepage}
  \begin{center}
	\includegraphics[width=0.5\textwidth]{unive.png}
	
    \vspace*{2cm}
    \huge
    \textmd{Computer Science}\\
    \large [CM9]

    \vspace{1.5cm}
    \huge Data Design and Nature-Inspired Computing\\
    
    \vspace{1cm}
    \line(1, 0){280}\\
    \vspace{1cm}
    \huge
    Homework 1\\
    \large $18^{th}$ October 2017

    \vfill

  \end{center}
  \begin{raggedright}
    \Large
    \textbf{Teaching Professor} \\
    \large Prof. Irene Poli\\
    
    \vspace{1cm}
    \Large
    \textbf{Author} \\
    \large 
    Feliks Hibraj\\
    Mat. 854342\\
    \vspace{0.5cm}
    \Large
    \textbf{Academic Year} \\
    \large 
    2018/2019\\

  \end{raggedright}
\end{titlepage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STILE HEADER - FOOTER - LISTE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\headheight}{14pt}

\pagestyle{fancy}
\lhead{}
\chead{}
\lhead{\textit{Homework 1}}
\rhead{\textbf{DDNC}}
\cfoot{}
\renewcommand{\headrulewidth}{0.4pt}
\renewcommand{\footrulewidth}{0.4pt}

\renewcommand{\labelitemi}{$\diamond$}
\renewcommand{\labelitemii}{$\bullet$}
\renewcommand{\labelitemiii}{$\circ$}

\setlist{itemsep=0pt}

\setlength{\parindent}{0cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% INDICE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagenumbering{gobble}
\renewcommand{\contentsname}{Index}
\tableofcontents
\newpage
\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOOTER CON NUMERO PAGINA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rfoot{\thepage\ di \pageref{LastPage}}


==> imgs/svgs/file.tex <==
\starttext
\externalfigure[test_wpbc.svg]
\stoptext

==> sec/abstract.tex <==
\newgeometry{top=2.5cm,bottom=1.5cm,right=3.5cm,left=3.5cm}
\begin{titlepage}
\huge
\begin{center}
\textbf{Abstract}
\end{center}
\vspace{1cm}
\large
Recently, classical kernel methods have been extended by the introduction of suitable tensor kernels so to promote sparsity in the solution of the underlying regression problem. Indeed they solve an \lp -norm regularization problem, with $p=m/(m-1)$ and $m$ even integer, which happens to be close to a lasso problem.
% In the end this may permit to expoit higher order dependencies between features.
However, a major drawback of the method is that storing tensors generally requires a considerable amount of memory, ultimately limiting its applicability. 
In this work we address this problem by proposing two advances.
First, we directly reduce the memory requirement, by introducing a new and more efficient layout for storing the data. 
Second, we use \nystrom-type subsampling approach, which allows for a training phase with a smaller number of data points, so to reduce the computational cost.
Experiments, both on synthetic and real datasets show the effectiveness of the proposed improvements.
Finally, we take care of implementing the code in $C++$ so to further speed-up the computation.
\newline
\bigbreak
\noindent
\begin{center}\textbf{Keywords}:\\\medbreak
\textit{Machine Learning, Tensor Kernels, Regularization, Optimization}
\end{center}
\end{titlepage}
\newgeometry{top=3.5cm,bottom=2.5cm,right=2.5cm,left=2.5cm}


==> sec/frontespizio.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TITOLO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagenumbering{Alph}
\begin{titlepage}
  \begin{center}
	\includegraphics[width=0.5\textwidth]{unive.png}
	
    \vspace*{2cm}
    \huge
    \textmd{Computer Science}\\
    \large [CM9]

    \vspace{1.5cm}
    \huge Data Design and Nature-Inspired Computing\\
    
    \vspace{1cm}
    \line(1, 0){280}\\
    \vspace{1cm}
    \huge
    Homework 1\\
    \large $18^{th}$ October 2017

    \vfill

  \end{center}
  \begin{raggedright}
    \Large
    \textbf{Teaching Professor} \\
    \large Prof. Irene Poli\\
    
    \vspace{1cm}
    \Large
    \textbf{Author} \\
    \large 
    Feliks Hibraj\\
    Mat. 854342\\
    \vspace{0.5cm}
    \Large
    \textbf{Academic Year} \\
    \large 
    2018/2019\\

  \end{raggedright}
\end{titlepage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STILE HEADER - FOOTER - LISTE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\headheight}{14pt}

\pagestyle{fancy}
\lhead{}
\chead{}
\lhead{\textit{Homework 1}}
\rhead{\textbf{DDNC}}
\cfoot{}
\renewcommand{\headrulewidth}{0.4pt}
\renewcommand{\footrulewidth}{0.4pt}

\renewcommand{\labelitemi}{$\diamond$}
\renewcommand{\labelitemii}{$\bullet$}
\renewcommand{\labelitemiii}{$\circ$}

\setlist{itemsep=0pt}

\setlength{\parindent}{0cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% INDICE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagenumbering{gobble}
\renewcommand{\contentsname}{Index}
\tableofcontents
\newpage
\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOOTER CON NUMERO PAGINA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rfoot{\thepage\ di \pageref{LastPage}}


==> sec/th_setup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TITOLO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagenumbering{Alph}
\begin{titlepage}
	\begin{center}
		\includegraphics[trim={0 9.7cm 5.75cm 0},clip,width=0.5\textwidth]{imgs/unive_logo.pdf}
				
		\vspace{1.5cm}
		\huge
		\textbf{Master's Degree in Computer Science}\\
		% \textbf{\titolo}\\
		\Large {[CM9] Computer Science - D.M. 270/2004}
		% \LARGE {\nome}
		
		\vspace{0.8cm}
		\Huge{Final Thesis}
		
    	\vspace{0.8cm}
		\Huge{\textbf{\thtitle}}\\
		\huge{\thsubtitle}
		\vspace{1cm}
		%\line(1, 0){280}\\
		\vfill
	\end{center}
  \begin{raggedright}
    \Large
    \textbf{Supervisors} \\
    \large Ch. Prof. Marcello Pelillo\\
    \large Ch. Prof. Massimiliano Pontil\\
    \vspace{0.5cm}
    \textbf{Advisor} \\
    \large Dott. Saverio Salzo\\
    \vspace{0.5cm}
    \Large
    \textbf{Graduand}\\ 
    \large 
    Feliks Hibraj \hfill {\Large \textbf{Academic Year}} \\
    Matriculation Number 854342 \hfill 2018/2019\\
    \vspace{0.5cm}
  \end{raggedright}
\end{titlepage}

\input{abstract.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STILE HEADER - FOOTER - LISTE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\headheight}{14pt}

\pagestyle{fancy}
\lhead{}
\chead{}
\lhead{\textit{\name}}
\rhead{\textbf{\headtitle}}
\cfoot{}
\renewcommand{\headrulewidth}{0.4pt}
\renewcommand{\footrulewidth}{0.4pt}

\renewcommand{\labelitemi}{$\circ$}
\renewcommand{\labelitemii}{$\bullet$}
\renewcommand{\labelitemiii}{$\diamond$}

\setlist{itemsep=0pt}

\setlength{\parindent}{0cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% INDICE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pagenumbering{gobble}
\renewcommand{\contentsname}{Index}
\tableofcontents
\newpage
\pagenumbering{arabic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FOOTER CON NUMERO PAGINA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rfoot{\thepage\ di \pageref{LastPage}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FUNZIONI
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\defi}[1]{\begin{mydef}{#1}\end{mydef}}
\newcommand{\defin}[2]{\begin{mydef}[#1]{#2}\end{mydef}}
\newcommand{\prop}[1]{\begin{myprop}{#1}\end{myprop}}
\newcommand{\lem}[1]{\begin{mylemma}{#1}\end{mylemma}}
\newcommand{\lemn}[2]{\begin{mylemma}[#1]{#2}\end{mylemma}}
\newcommand{\thm}[1]{\begin{mytheorem}{#1}\end{mytheorem}}
\newcommand{\thmn}[2]{\begin{mytheorem}[#1]{#2}\end{mytheorem}}

\newcommand{\spa}{\vspace*{0.35cm}}




